Exact Inference for Stochastic Epidemic Models via Uniformly Ergodic Block Sampling

Stochastic epidemic models provide an interpretable probabilistic description of the spread of a disease through a population. Yet, fitting these models to partially observed data is a notoriously difficult task due to intractability of the likelihood for many classical models. To remedy this issue, this article introduces a novel data-augmented MCMC algorithm for exact Bayesian inference under the stochastic SIR model, given only discretely observed counts of infection. In a Metropolis-Hastings step, the latent data are jointly proposed from a surrogate process carefully designed to closely resemble the SIR model, from which we can efficiently generate epidemics consistent with the observed data. This yields a method that explores the high-dimensional latent space efficiently, and scales to outbreaks with hundreds of thousands of individuals. We show that the Markov chain underlying the algorithm is uniformly ergodic, and validate its performance via thorough simulation experiments and a case study on the 2013-2015 outbreak of Ebola Haemorrhagic Fever in Western Africa.

==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
